Raw Report on the Model Checking Contest at Petri Nets 2012

This article presents the results of the Model Checking Contest held at Petri Nets 2012 in Hambourg. This contest aimed at a fair and experimental evaluation of the performances of model checking techniques applied to Petri nets. This is the second edition after a successful one in 2011. The participating tools were compared on several examinations (state space generation and evaluation of several types of formulae - structural, reachability, LTL, CTL) run on a set of common models (Place/Transition and Symmetric Petri nets). After a short overview of the contest, this paper provides the raw results from the context, model per model and examination per examination.

==> Makefile <==
MAINLATEX	=	"MCC-report"

build:
	pdflatex MCC-report.tex
	bibtex MCC-report
	pdflatex MCC-report.tex
	pdflatex MCC-report.tex


# all: plot
# 	pdflatex $(MAINLATEX).tex
# 	bibtex $(MAINLATEX)
# 	pdflatex $(MAINLATEX).tex
# 	pdflatex $(MAINLATEX).tex
# 	latex $(MAINLATEX).tex
# 	sh -c 'case `uname -s` in \
# 					 "Darwin") open $(MAINLATEX).pdf ;; \
# 					 "Linux") xpdf $(MAINLATEX).pdf & ;; \
# 					 *) ;; \
# 				 esac'
# 
# plot:
# 	sh generate-charts.sh
# 
# clean:
# 	rm -f MCC-report.pdf
# 	rm -f MCC-report.aux MCC-report.bbl MCC-report.blg MCC-report.cb MCC-report.cb2 MCC-report.dvi MCC-report.fdb_latexmk MCC-report.fls MCC-report.log MCC-report.out MCC-report.synctex.gz
# 	rm -f *~
# 	rm -f sections/*/*.eps sections/*/*-eps-converted-to.pdf


==> includes/content_state_space_ko.tex <==
\begin{itemize} 
\item cs\_repetitions, 
\item neo-election, 
\item planning, 
\end{itemize} 


==> includes/macros-al.tex <==
\makeatletter
\define@choicekey*{result}{reached}[\val\nr]{nc,none,some,best,max}{%
\ifcase\nr\relax%
  \gdef\result@line{}%
  \cellcolor{white}%
\or%
  \gdef\result@number{}%
  \cellcolor{gray!50}%
\or%
  \cellcolor{gray!90}%
\or%
  \cellcolor{black!70}%
  \color{white}%
\or%
  \cellcolor{black}%
  \color{white}%
\fi%
}
\define@choicekey*{result}{typepn}[\val\nr]{no,pt,cn}{%
\ifcase\nr\relax%
  \gdef\result@line{}%
\or%
  \gdef\result@line{\hfill P}%
\or%
  \gdef\result@line{\hfill C}%
\fi%
}
\newcommand\result[2][]{%
  \gdef\result@number{#2}
  \setkeys{result}{#1}%
  \result@number\result@line%
}
\newcommand\legend{%
{%
  \scriptsize
  \begin{tabular}{|p{4em}|cl}
  \cline{1-1}
    \cellcolor{white}
    & & The tool does not participate.
    \\
    \cellcolor{gray!50}
    & & The tool participates, but cannot compute for any scaling value.
    \\
    \cellcolor{gray!90}
    & & The tool participates.
    \\
    \cellcolor{black!70}
    & & The tool participates and reaches the best parameter among tools.
    \\
    \cellcolor{black}
    & & The tool participates and reaches the maximum parameter.
    % \\
    % %$n$ \hfill T
    % & & The tool failed.
%     \\
%     $n$ \hfill 
%     & & The tool fails because of memory exhaustion, after reaching parameter~$n$.
%     \\
% %    $n$ \hfill \Laserbeam
% %    & & The tool fails because of stack overflow, after reaching parameter~$n$.
% %    \\
%     $n$ \hfill \Clocklogo
%     & & The tool fails because of maximum time is elapsed, after reaching parameter~$n$.
    \\
  \cline{1-1}
\end{tabular}
}%
}
\makeatother

